An enhanced method with local energy minimization for the robust a posteriori construction of equilibrated stress fields in finite element analyses

In the context of global/goal-oriented error estimation applied to computational mechanics, the need to obtain reliable and guaranteed bounds on the discretization error has motivated the use of residual error estimators. These estimators require the construction of admissible stress fields verifying the equilibrium exactly. This article focuses on a recent method, based on a flux-equilibration procedure and called the element equilibration + star-patch technique (EESPT), that provides for such stress fields. The standard version relies on a strong prolongation condition in order to calculate equilibrated tractions along finite element boundaries. Here, we propose an enhanced version, which is based on a weak prolongation condition resulting in a local minimization of the complementary energy and leads to optimal tractions in selected regions. Geometric and error estimate criteria are introduced to select the relevant zones for optimizing the tractions. We demonstrate how this optimization procedure is important and relevant to produce sharper estimators at affordable computational cost, especially when the error estimate criterion is used. Two- and three-dimensional numerical experiments demonstrate the efficiency of the improved technique.

==> pdfsync.tex <==
%%%%  This is pdfsync.tex
%%%%  Ascii text file
%%%%  2004-01-20:
%%%%
%%%%  Version 0.1 usage: \input pdfsync.tex
%%%%  ============================
%%%%  appends reference points before each \par and at each \hbox, inline math;
%%%%  Known commands:
%%%%  \pdfsync: add this command everywhere you want to reference a point
%%%%  \pdfsyncstop, \pdfsyncstart: if pdfsync beaks your code, enclose the dangerous part in stop start group
%%%%
%%%%  THIS IS NOT COMPATIBLE WITH \input
%%%%  USE THE \import{foo} syntax whenever you want to import a file.
%%%%  Credits:
%%%%  ========
%%%%  This file is due to Piero D'Ancona and jlaurens@users.sourceforge.net
%%%%  iTeXMac and TeXShop are supporting pdfsync
%%%%  Copy this file to ~/Library/texmf/tex/plain or ~/Library/TeX/texmf/tex/plain if available
%%%%  This file is distributed under the GPL and the "smart licence": please make things better if you can
%%%%  copyright 2004, jlaurens@users.sourceforge.net
%
\catcode`\@11\relax
\newif\ifPDFSYNCOK%
\newif\ifPDFSYNCStar%
\newif\ifPDFSYNCPar\PDFSYNCPartrue%
\newif\ifPDFSYNCMath\PDFSYNCMathtrue%
\newif\ifPDFSYNCHBox\PDFSYNCHBoxtrue%
\newif\ifPDFSYNCExtra\PDFSYNCExtratrue%
\newif\ifPDFSYNCOn\PDFSYNCOntrue%
\newwrite\PDFPOS%
\newcount\PDFSYNC@folio\PDFSYNC@folio=0%
\newcount\PDFSYNC@rder\PDFSYNC@rder=0%
\ifx\pdfsavepos\undefined%
  \wlog{****  pdfsync.tex: Synchronization is only available with pdf. Use a dvi viewer instead.}%
  \let\pdfsyncstart\relax%
  \let\pdfsyncstop\relax%
  \let\pdfsync\relax%
  \let\@PDFSYNC\relax%
\else%
 \def\pdfsyncstart{\global\PDFSYNCOKtrue}%
  \def\pdfsyncstop{\global\PDFSYNCOKfalse}%
  \def\configure@PDFSYNC{%
  \ifPDFSYNCOn%
    \wlog{****  pdfsync.tex: Synchronization is enabled.}%
    \immediate\openout\PDFPOS\jobname.pdfsync%
    \immediate\write\PDFPOS{\jobname}%            control info
    \immediate\write\PDFPOS{version 0}%            control info
	\global\advance\PDFSYNC@folio by 1\relax
	\immediate\write\PDFPOS{s\space\the\PDFSYNC@folio}
   % patching plain \advancepageno
	\global\let\PDFSYNC@advancepageno\advancepageno%
	\gdef\advancepageno{%
	\global\advance\PDFSYNC@folio by 1\relax
		\immediate\write\PDFPOS{s\space\the\PDFSYNC@folio}
	\PDFSYNC@advancepageno
	}%
   % new command to import
    \def\import##1{%
	  \immediate\write\PDFPOS{(##1}%
      \input ##1%
      \immediate\write\PDFPOS{)}}%
    \def\@PDFSYNC{%
    \relax
    \ifPDFSYNCOK
	\pdfsavepos
	\immediate\write\PDFPOS{l\space\the\PDFSYNC@rder\space\the\inputlineno}%
	\def\PDFSYNC@position{\the\pdflastxpos\space\the\pdflastypos}%
	\ifPDFSYNCStar%
	    \edef\argument%
		    {{p*\space\the\PDFSYNC@rder\space\noexpand\PDFSYNC@position}}%
	\else%
	    \edef\argument%
		    {{p\space\the\PDFSYNC@rder\space\noexpand\PDFSYNC@position}}%
	\fi%
	\expandafter\write\expandafter\PDFPOS\argument%
	\global\advance\PDFSYNC@rder by 1%
    \fi\relax}%
    \ifPDFSYNCPar\wlog{****  pdfsync.tex: Synchronizing par}%
	    \global\let\PDFSYNC@par\par\gdef\par{\PDFSYNC@par\@PDFSYNC}\fi%
    \ifPDFSYNCMath\wlog{****  pdfsync.tex: Synchronizing math}%
	    \everymath{\@PDFSYNC\relax}\fi%
    \ifPDFSYNCHBox\wlog{****  pdfsync.tex: Synchronizing hbox}%
	    \everyhbox{\@PDFSYNC}\fi%
%	    \everyhbox{\aftergroup\@PDFSYNC\relax}\fi%
    \def\pdfsync{\global\PDFSYNCStartrue\@PDFSYNC\global\PDFSYNCStarfalse}%
  \else%
    \wlog{****  pdfsync.tex: Synchronization is disabled.}%
    \let\pdfsyncstart\relax%
    \let\pdfsyncstop\relax%
    \let\pdfsync\relax%
    \let\@PDFSYNC\relax%  
  \fi%
  }%
 \def\PDFSYNC@Extra{}%
\pdfsyncstart%
\configure@PDFSYNC%
\fi
\catcode`\@12\relax
\endinput


==> pdfsync4context.tex <==
%%%%  This is pdfsync4context.tex
%%%%  Ascii text file
%%%%  2004-01-31: Version 0.2
%%%%  - The pdfsync anchor is used after the \par
%%%%  2004-01-20:
%%%%  THIS IS BETA SOFTWARE
%%%%  Version 0.2 usage: \input pdfsync4context.tex
%%%%  ============================
%%%%  appends reference points before each \par and at each \hbox, inline math;
%%%%  Known commands:
%%%%  \pdfsync: add this command everywhere you want to reference a point
%%%%  \pdfsyncstop, \pdfsyncstart: if pdfsync beaks your code, enclose the dangerous part in stop start group
%%%%
%%%%  THIS IS NOT COMPATIBLE WITH \input
%%%%  USE THE STANDARD CONTEXT CODE TO READ FILES.
%%%%  Credits:
%%%%  ========
%%%%  This file is due to Piero D'Ancona and jlaurens@users.sourceforge.net
%%%%  iTeXMac and TeXShop are supporting pdfsync
%%%%  Copy this file to ~/Library/texmf/tex/plain or ~/Library/TeX/texmf/tex/plain if available
%%%%  This file is distributed under the GPL and the "smart licence": please make things better if you can
%%%%  copyright 2004, jlaurens@users.sourceforge.net (Sat Jan 24 09:42:35 GMT 2004)
%
\wlog{****  This pdfsync4context.tex version 0.2.}%
\catcode`\@11\relax%
\ifx\pdfsavepos\undefined%
    \wlog{****  pdfsync4context.tex: Synchronization is only available with pdf. Use a dvi viewer instead.}%
    \let\pdfsyncstart\relax%
    \let\pdfsyncstop\relax%
    \let\pdfsync\relax%
    \let\@PDFSYNC\relax%
\else%
    \wlog{****  pdfsync4context.tex: Synchronization is available.}%
    \newif\ifPDFSYNCOK%
    \newif\ifPDFSYNCStar%
    \newcount\PDFSYNC@folio\PDFSYNC@folio=0%
    \newcount\PDFSYNC@rder\PDFSYNC@rder=0%
    \gdef\pdfsyncstart{\PDFSYNCOKtrue}%
    \gdef\pdfsyncstop{\PDFSYNCOKfalse}%
    \wlog{****  pdfsync.tex: configuring synchronization.}%
    \newwrite\PDFPOS%
    \immediate\openout\PDFPOS\jobname.pdfsync%
    \immediate\write\PDFPOS{\jobname}%            control info
    \immediate\write\PDFPOS{version 0}%            control info
    % patching \shipout
    \global\let\PDFSYNC@oldshipout\shipout%
    \gdef\shipout#1{%
        \global\advance\PDFSYNC@folio by 1\relax%
        \immediate\write\PDFPOS{s\space\the\PDFSYNC@folio}%
        \PDFSYNC@oldshipout#1}%
    \gdef\PDFSYNC@position{\the\pdflastxpos\space\the\pdflastypos}%
    \gdef\@PDFSYNC{%
%        \relax%
        \ifPDFSYNCOK%
            \pdfsavepos%
            \immediate\write\PDFPOS{l\space\the\PDFSYNC@rder\space\the\inputlineno}%
            \ifPDFSYNCStar%
                \edef\argument%
                    {{p*\space\the\PDFSYNC@rder\space\noexpand\PDFSYNC@position}}%
            \else%
                \edef\argument%
                    {{p\space\the\PDFSYNC@rder\space\noexpand\PDFSYNC@position}}%
            \fi%
            \expandafter\write\expandafter\PDFPOS\argument%
            \global\advance\PDFSYNC@rder by 1%
        \fi%\relax%
    }%
    \wlog{****  pdfsync.tex: Synchronizing par}%
    \global\let\PDFSYNC@par\par%
    \gdef\par{\PDFSYNC@par\@PDFSYNC}%
    \wlog{****  pdfsync.tex: Synchronizing math}%
    \everymath{\@PDFSYNC\relax}%
    \wlog{****  pdfsync.tex: Synchronizing hbox}%
    \everyhbox{\@PDFSYNC\relax}%
    \def\pdfsync{\global\PDFSYNCStartrue\@PDFSYNC\global\PDFSYNCStarfalse}%
    \def\PDFSYNC@begin{\immediate\write\PDFPOS{(\space\readfilename}}%
    \def\PDFSYNC@end{\immediate\write\PDFPOS{)}}%
    \appendtoks\PDFSYNC@begin\to\everybeforereadfile%
    \appendtoks\PDFSYNC@end\to\everyafterreadfile%
    \pdfsyncstart%
    \wlog{****  pdfsync.tex: BUG WARNING, DID YOU LOOK AT THE README?}%
\fi%
\catcode`\@12\relax%
\endinput%

